Continuous $-1$ Hypergeometric Orthogonal Polynomials

The study of $-1$ orthogonal polynomials viewed as $q =-1$ limits of the $q$-orthogonal polynomials is pursued. This paper present the continuous polynomials part of the $-1$ analog of the $q$-Askey scheme. A compendium of the properties of all the continuous $-1$ hypergeometric polynomials and their connections is provided.

==> Sections/BI.tex <==
\subsection{Bannai-Ito}
\textbf{\textit{\large Hypergeometric Representation}}\\
\begin{gather}
    \frac{\mathbf{B}_{2n}\left(x;\rho_1,\rho_2,r_1,r_2\right)}{N_{2n}} = \pFq{4}{3}{-n,n+g+1,x-r_1+\frac{1}{2},-x+r_1+\frac{1}{2}}{1-r_1-r_2,\rho_1-r_1+\frac{1}{2},\rho_2-r_1+\frac{1}{2}}{1}+\qquad \label{BIBHR1} \\
    \xi_{2n}\left(x-r_1+\frac{1}{2}\right)\pFq{4}{3}{-n+1,n+g+1,x-r_1+\frac{3}{2},-x+r_1+\frac{1}{2}}{1-r_1-r_2,\rho_1-r_1+\frac{3}{2},\rho_2-r_1+\frac{3}{2}}{1} \nonumber\\[0.5cm]
    \frac{\mathbf{B}_{2n+1}\left(x;\rho_1,\rho_2,r_1,r_2\right)}{N_{2n+1}} = \frac{-1}{\eta_{2n+1}}\pFq{4}{3}{-n,n+g+1,x-r_1+\frac{1}{2},-x+r_1+\frac{1}{2}}{1-r_1-r_2,\rho_1-r_1+\frac{1}{2},\rho_2-r_1+\frac{1}{2}}{1}+\qquad\label{BIBHR2}\\
    \left(x-r_1+\frac{1}{2}\right)\pFq{4}{3}{-n,n+g+2,x-r_1+\frac{3}{2},-x+r_1+\frac{1}{2}}{1-r_1-r_2,\rho_1-r_1+\frac{3}{2},\rho_2-r_1+\frac{3}{2}}{1} \nonumber
\end{gather}
Where
\begin{gather}
    g=\rho_1+\rho_2-r_1-r_2\\[0.5cm]
    \xi_{2n}=\frac{n}{\left(\rho_1-r_1+\frac{1}{2}\right)\left(\rho_2-r_1+\frac{1}{2}\right)}\qquad  N_{2n}=\frac{\poch{1-r_1-r_2}{n} \poch{\rho_1-r_1+\frac{1}{2}}{n} \poch{\rho_2-r_1+\frac{1}{2}}{n}}{\poch{n+g+1}{n}} \\[0.5cm]
    \eta_{2n+1}=\frac{n+g+1}{\left(\rho_1-r_1+\frac{1}{2}\right)\left(\rho_2-r_1+\frac{1}{2}\right)}\quad N_{2n+1}=\frac{\poch{1-r_1-r_2}{n} \poch{\rho_1-r_1+\frac{3}{2}}{n} \poch{\rho_2-r_1+\frac{3}{2}}{n}}{\poch{n+g+2}{n}}\qquad
\end{gather}
\textbf{\textit{\large Orthogonality Relation}}\\
There are four truncation conditions when $N$ is even and two when $N$ is odd. For each combination of truncation condition, there is an orthogonality relation. \\
\begin{gather}
    \sum_{s=0}^{N} \widetilde{w}_{s} \mathbf{B}_{n}\left(x_{s}\right) \mathbf{B}_{m}\left(x_{s}\right)=\left(\sum_{s=0}^{N} \widetilde{w}_{s}\right)\left(\prod_{k=1}^{n} \tau_k\right) \delta_{n m}\\[0.3cm]
    w_{s}\left(\rho_{1}, \rho_{2}, r_{1}, r_{2}\right)=\frac{(-1)^{\nu}}{\ell !} \frac{\left(\rho_{1}-r_{1}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}-r_{2}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}+\rho_{2}+1\right)_{\ell}\left(2 \rho_{1}+1\right)_{\ell}}{\left(\rho_{1}+r_{1}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}+r_{2}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}-\rho_{2}+1\right)_{\ell}}
\end{gather}Where $s=2l+\nu,\quad \nu\in\{0,1\}$. \\[0.5cm]
1. For $r_{1}=\frac{N+1}{2}+\rho_{1}, r_{2}=\frac{N+1}{2}+\rho_{1}$ with $N$ even:
$$
x_{s}=(-1)^{s}\left(\rho_{1}+s / 2+1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}= w_{s}\left(\rho_{1}, \rho_{2}, r_{1}, r_{2}\right)
$$
2. For $r_{1}=\frac{N+2}{2}+\rho_{2}$ or $r_{2}=\frac{N+1}{2}+\rho_{2}$ with $N$ even:
$$
x_{s}=(-1)^{s}\left(\rho_{2}+s / 2+1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}= w_{s}\left(\rho_{2}, \rho_{1}, r_{1}, r_{2}\right)
$$
3. For $\rho_{1}+\rho_{2}=-\frac{N+1}{2}$ with $N$ odd:
$$
x_{s}=(-1)^{s}\left(\rho_{2}+s / 2+1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}= w_{s}\left(\rho_{2}, \rho_{1}, r_{1}, r_{2}\right)
$$
4. For $r_{1}+r_{2}=\frac{N+1}{2}$ with $N$ odd:
$$
x_{s}=(-1)^{s}\left(r_{1}-s / 2-1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}= w_{s}\left(-r_1,-r_2,-\rho_{1}, -\rho_{2}\right)
$$

\textbf{\textit{\large Normalized recurrence relation}}\\
\begin{gather}
    x\mathbf{B}_n(x) = \mathbf{B}_{n+1}(x) + \left(\rho_1-A_n-C_n\right)\mathbf{B}_n(x) + A_{n-1}C_n \mathbf{B}_{n-1}(x)
\end{gather}
\begin{minipage}{.45\textwidth}
        \begin{eqnarray}
    A_{n}=\left\{\begin{array}{ll}
\frac{\left(n+1+2\rho_1-2r_1\right)\left(n+1+2\rho_1-2r_2\right)}{4\left(n+1+g\right)}&n\text{ even}\\[0.15cm]
\frac{\left(n+1+2g\right)\left(n+1+2\rho_1+2\rho_2\right)}{4\left(n+1+g\right)}& n\text{ odd}
\end{array}\right.\nonumber
\end{eqnarray}
    \end{minipage}%
    \begin{minipage}{0.55\textwidth}
       \begin{eqnarray}
   C_{n}=\left\{\begin{array}{ll}
\frac{-n\left(n-2r_1-2r_2\right)}{4\left(n+g\right)}&n\text{ even}\\[0.15cm]
\frac{-\left(n+2\rho_2-2r_2\right)\left(n+2\rho_2-2r_1\right)}{4\left(n+g\right)}& n\text{ odd}
\end{array}\right.\label{BIRRC}
\end{eqnarray}
    \end{minipage}\\[0.3cm]


\textbf{\textit{\large Difference Equation}}\\
\begin{gather}
    \left(F(x)\left[I-R\right]+G(x)\left[T^+ R-I\right]\right)\mathbf{B}_n(x)=\lambda_n \mathbf{B}_n(x)\\[0.3cm]
    F(x)=\frac{\pp{x-\rho_1}\pp{x-\rho_2}}{2x} \qquad G(x)=\frac{\pp{x-r_1+\frac{1}{2}}\pp{x-r_2+\frac{1}{2}}}{2x+1}\\[0.3cm]
    \lambda_{n}=\left\{\begin{array}{ll}
\frac{n}{2}&n\text{ even}\\[0.15cm]
-g-\frac{n+1}{2}& n\text{ odd}\end{array}\right.
\end{gather}

\textbf{\textit{\large Limit Relations}}\\[0.5cm]
\textbf{\textit{\large Askey-Wilson $\to$ Bannai-Ito}}\\[0.3cm]
The Bannai-Ito polynomials are obtained from the monic Askey-Wilson polynomials by taking the parametrization $q=-e^\varepsilon$, $a=-ie^{\varepsilon(2\rho_1+\frac{1}{2})}$, $b=-ie^{\varepsilon(2\rho_2+\frac{1}{2})}$, $c=ie^{\varepsilon(-2r_2+\frac{1}{2})}$, $d=ie^{\varepsilon(-2r_1+\frac{1}{2})}$, $z=ie^{-\varepsilon(2y+\frac{1}{2})}$ and $x=(z+z^{-1})/2$.
\begin{gather}
    \lim\limits_{\varepsilon\to0}\mathbf{P}_n\left(x(z);a,b,c,d|q\right)=\mathbf{B}_n\left(y;\rho_1,\rho_2,r_1,r_2\right)
\end{gather}





\textbf{\textit{\large Bannai-Ito $\to$ Complementary Bannai-Ito}}\\[0.3cm]
The Complementary Bannai-Ito polynomials are obtained by the Christoffel transformation of the Bannai-Ito polynomials and vice-versa via the Geronimus transformation. 
\begin{gather}
    \mathbf{I}_{n}(x)=\frac{\mathbf{B}_{n+1}(x)-A_{n} \mathbf{B}_{n}(x)}{x-\rho_{1}}\qquad \mathbf{B}_{n}(x)=\mathbf{I}_{n}(x)-C_{n} \mathbf{I}_{n-1}(x) 
\end{gather}
Where $A_n$ and $C_n$ are given by \eqref{BIRRC}. 




\textbf{\textit{\large Bannai-Ito $\to$ Continuous Bannai-Ito}}\\[0.3cm]
The Bannai-Ito polynomials and the Continuous Bannai-Ito polynomials are related in the following way.
\begin{gather}
    \mathbf{Q}_n\left(x;\alpha,\beta,\gamma,\delta\right) = (-2i)^n \mathbf{B}_n\left(i\left(\frac{x}{2}-\frac{1}{4}\right);\alpha+i\beta+\frac{1}{4},\gamma+i\delta+\frac{1}{4},-\alpha+i\beta-\frac{1}{4},-\gamma+i\delta-\frac{1}{4}\right)
\end{gather}

\textbf{\textit{\large Bannai-Ito $\to$ Big -1 Jacobi}}\\[0.3cm]
The Big -1 Jacobi polynomial given by \eqref{B-1JBHR1},\eqref{B-1JBHR2} can be obtained from the Bannai-Ito polynomials using the parametrization $x\to\frac{x}{h}$, $\rho_1\to\frac{\beta}{2}-\frac{c}{h}$, $\rho_2\to\frac{\alpha}{2}+\frac{1}{h}$, $r_1\to-\frac{c}{h}$ and $r_1\to\frac{1}{h}$ in \eqref{BIBHR1},\eqref{BIBHR2} and taking the limit $h\to0$.
\begin{gather}
    \lim\limits_{h\to0}\mathbf{B}_n\left(\frac{x}{h};\frac{\beta}{2}-\frac{c}{h},\frac{\alpha}{2}+\frac{1}{h},-\frac{c}{h},\frac{1}{h}\right) = \mathbf{J}_n\left(x;\alpha,\beta,c\right)
\end{gather}

==> Sections/CBI.tex <==
\subsection{Complementary Bannai-Ito}
\textbf{\textit{\large Hypergeometric Representation}}\\
\begin{gather}
    \mathbf{I}_{2n}\left(x;\rho_1,\rho_2,r_1,r_2\right) = \eta_{2n}\pFq{4}{3}{-n,n+g+1,\rho_2+x,\rho_2-x}{1+\rho_1+\rho_2,\rho_2-r_1+\frac{1}{2},\rho_2-r_2+\frac{1}{2}}{1} \label{CBIBHR1}\\[0.5cm]
    \mathbf{I}_{2n+1}\left(x;\rho_1,\rho_2,r_1,r_2\right) = \eta_{2n+1}(x-\rho_2)\pFq{4}{3}{-n,n+g+2,\rho_2+x+1,\rho_2-x+1}{2+\rho_1+\rho_2,\rho_2-r_1+\frac{3}{2},\rho_2-r_2+\frac{3}{2}}{1}\label{CBIBHR2}
\end{gather}
Where
\begin{gather}
    g=\rho_1+\rho_2-r_1-r_2\\[0.5cm]
     \eta_{2n}=\frac{\poch{1+\rho_1+\rho_2}{n} \poch{\rho_2-r_1+\frac{1}{2}}{n} \poch{\rho_2-r_2+\frac{1}{2}}{n}}{\poch{n+g+1}{n}} \\[0.5cm]
     \eta_{2n+1}=\frac{\poch{2+\rho_1+\rho_2}{n} \poch{\rho_2-r_1+\frac{3}{2}}{n} \poch{\rho_2-r_2+\frac{3}{2}}{n}}{\poch{n+g+2}{n}}
\end{gather}
\textbf{\textit{\large Orthogonality Relation}}\\
There are three truncation conditions when $N$ is even and three when $N$ is odd. For each combination of truncation condition, there is an orthogonality relation. \\
\begin{gather}
    \sum_{s=0}^{N} \widetilde{w}_{s} \mathbf{I}_{n}\left(x_{s}\right) \mathbf{I}_{m}\left(x_{s}\right)=\left(\sum_{s=0}^{N} \widetilde{w}_{s}\right)\left(\prod_{k=1}^{n} \tau_k\right) \delta_{n m}\\[0.3cm]
    w_{s}\left(\rho_{1}, \rho_{2}, r_{1}, r_{2}\right)=\frac{(-1)^{\nu}}{\ell !} \frac{\left(\rho_{1}-r_{1}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}-r_{2}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}+\rho_{2}+1\right)_{\ell}\left(2 \rho_{1}+1\right)_{\ell}}{\left(\rho_{1}+r_{1}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}+r_{2}+1 / 2\right)_{\ell+\nu}\left(\rho_{1}-\rho_{2}+1\right)_{\ell}}
\end{gather}Where $s=2l+\nu,\quad \nu\in\{0,1\}$. \\[0.5cm]
1. For $r_{1}=\frac{N+1}{2}+\rho_{2}, r_{2}=\frac{N+1}{2}+\rho_{2}$ or $\rho_{1}=-\frac{N+2}{2}-\rho_{2}$ with $N$ even:
$$
x_{s}=(-1)^{s}\left(\rho_{2}+s / 2+1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}=\left(x_{s}-\rho_{1}\right) w_{s}\left(\rho_{2}, \rho_{1}, r_{1}, r_{2}\right)
$$
2. For $r_{1}=\frac{N+2}{2}+\rho_{1}$ or $r_{1}=\frac{N+1}{2}-r_{2}$ with $N$ odd:
$$
x_{s}=(-1)^{s}\left(r_{1}-s / 2-1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}=\left(x_{s}-\rho_{1}\right) w_{s}\left(-r_{1},-r_{2},-\rho_{1},-\rho_{2}\right)
$$
3. For $r_{2}=\frac{N+2}{2}+\rho_{1}$ with $N$ odd:
$$
x_{s}=(-1)^{s}\left(r_{2}-s / 2-1 / 4\right)-1 / 4, \quad \widetilde{w}_{s}=\left(x_{s}-\rho_{1}\right) w_{s}\left(-r_{2},-r_{1},-\rho_{1},-\rho_{2}\right) .
$$



\textbf{\textit{\large Normalized recurrence relation}}\\
\begin{gather}
    x \mathbf{I}_{n}(x)=\mathbf{I}_{n+1}(x)+(-1)^{n} \rho_{2} \mathbf{I}_{n}(x)+\tau_{n} \mathbf{I}_{n-1}(x)\\[0.3cm]
    \begin{array}{l}
\tau_{2 n}=-\frac{n\left(n+\rho_{1}-r_{1}+1 / 2\right)\left(n+\rho_{1}-r_{2}+1 / 2\right)\left(n-r_{1}-r_{2}\right)}{(2 n+g)(2 n+g+1)}, \\[0.3cm]
\tau_{2 n+1}=-\frac{(n+g+1)\left(n+\rho_{1}+\rho_{2}+1\right)\left(n+\rho_{2}-r_{1}+1 / 2\right)\left(n+\rho_{2}-r_{2}+1 / 2\right)}{(2 n+g+1)(2 n+g+2)}
\end{array}
\end{gather}


\textbf{\textit{\large Difference Equation}}\\
\begin{gather}
    L^{(\alpha)}\mathbf{I}_n(x) = \Lambda^{(\alpha)}\mathbf{I}_n(x)\\[0.3cm]
   L^{(\alpha)} = A(x) T^{+}+B(x) T^{-}+C(x) R+D(x) T^{+} R+\alpha \frac{\left(x-\rho_{2}\right)}{2 x}(\mathbb{I}-R) \nonumber\\\qquad\qquad-(A(x)+B(x)+C(x)+D(x)) \mathbb{I}
\end{gather}
Where 
\begin{gather}
    \begin{array}{l}
A(x)=\frac{\left(x+\rho_{1}+1\right)\left(x+\rho_{2}+1\right)\left(2 x-2 r_{1}+1\right)\left(2 x-2 r_{2}+1\right)}{8(x+1)(2 x+1)} \\
B(x)=\frac{\left(x-\rho_{2}\right)\left(x-\rho_{1}-1\right)\left(2 x+2 r_{1}-1\right)\left(2 x+2 r_{2}-1\right)}{8 x(2 x-1)} \\
C(x)=\frac{\left(x-\rho_{2}\right)\left(4 x^{2}+\omega\right)}{8 x}-\frac{\left(x-\rho_{2}\right)\left(x+\rho_{1}+1\right)\left(2 x-2 r_{1}+1\right)\left(2 x-2 r_{2}+1\right)}{8 x(2 x+1)}-B(x) \\
D(x)=\frac{\rho_{2}\left(x+\rho_{1}+1\right)\left(2 x-2 r_{1}+1\right)\left(2 x-2 r_{2}+1\right)}{8 x(x+1)(2 x+1)}
\end{array}
\end{gather}
With
\begin{gather}
    \omega=4 \rho_{1}-4\left(r_{1}+r_{2}\right) \rho_{1}+4 r_{1} r_{2}-6\left(r_{1}+r_{2}\right)+5
\end{gather}
And
\begin{gather}
    \Lambda_{2 n}^{(\alpha)}=n^{2}+(g+1) n, \quad \Lambda_{2 n+1}^{(\alpha)}=n^{2}+(g+2) n+\alpha
\end{gather}
Using one of the grid of the orthogonality relation, we can show that this difference operator $L^{(\alpha)}$ correspond to a pentadiagonal operator when using the Complementary Bannai-Ito polynomials as a basis\cite{Genest_2013}. 


\textbf{\textit{\large Limit Relations}}\\[0.3cm]

\textbf{\textit{\large Askey-Wilson $\to$ Complementary Bannai-Ito}}\\[0.3cm]
The Bannai-Ito polynomials are obtained from the monic Askey-Wilson polynomials by taking the parametrization $q=-e^\varepsilon$, $a=ie^{\varepsilon(2\rho_1+\frac{3}{2})}$, $b=-ie^{\varepsilon(2\rho_2+\frac{1}{2})}$, $c=ie^{\varepsilon(-2r_2+\frac{1}{2})}$, $d=ie^{\varepsilon(-2r_1+\frac{1}{2})}$, $z=ie^{-\varepsilon(2y+\frac{1}{2})}$ and $x=(z+z^{-1})/2$.
\begin{gather}
    \lim\limits_{\varepsilon\to0}\mathbf{P}_n\left(x(z);a,b,c,d|q\right)=\mathbf{I}_n\left(y;\rho_1,\rho_2,r_1,r_2\right)
\end{gather}

\textbf{\textit{\large Bannai-Ito $\to$ Complementary Bannai-Ito}}\\[0.3cm]
The Complementary Bannai-Ito polynomials are obtained by the Christoffel transformation of the Bannai-Ito polynomials and vice-versa via the Geronimus transformation. 
\begin{gather}
    \mathbf{I}_{n}(x)=\frac{\mathbf{B}_{n+1}(x)-A_{n} \mathbf{B}_{n}(x)}{x-\rho_{1}}\qquad \mathbf{B}_{n}(x)=\mathbf{I}_{n}(x)-C_{n} \mathbf{I}_{n-1}(x) 
\end{gather}
Where $A_n$ and $C_n$ are given by \eqref{BIRRC}.


\textbf{\textit{\large Complementary Bannai-Ito $\to$ Chihara}}\\[0.3cm]
The Chihara polynomials given by \eqref{CBHR1},\eqref{CBHR2} can be obtained from the Complementart Bannai-Ito polynomials using the parametrization $x\to\frac{x\sqrt{a_1^2-a_2^2}}{h}$, $\rho_1\to\frac{a_1}{h}+b_1$, $\rho_2\to\frac{a_2}{h}+b_2$, $r_1\to\frac{a_1}{h}$ and $r_2\to\frac{a_2}{h}$ in \eqref{CBIBHR1},\eqref{CBIBHR2} and taking the limit $h\to0$. Finally, using $\alpha=b_2-\frac{1}{2}$, $\beta=b_1+\frac{1}{2}$ and $\gamma=\frac{a_2}{\sqrt{a_1^2-a_2^2}}$, we get the Chihara polynomial.
\begin{gather}
    \lim\limits_{h\to0}\mathbf{I}_n\left(\frac{x}{h};\frac{a_1}{h}+b_1,\frac{a_2}{h}+b_2,\frac{a_1}{h},\frac{a_2}{h}\right) = \mathbf{C}_n\left(x;\alpha,\beta,\gamma\right)
\end{gather}





==> dia/dia2.tex <==
\begin{center}
\adjustbox{max width=12cm}{\begin{tikzpicture}[>=stealth,->,shorten >=2pt,looseness=.5,auto]
\matrix [matrix of math nodes,
column sep={6cm,between origins},
row sep={4cm,between origins}]
{
|(21)| \begin{tabular}{c} \( \text{Chihara} \) \\ \( C_n(x;\alpha,\beta,\gamma) \) \end{tabular} & |(22)|  \begin{tabular}{c} \( \text{Big q-Jacobi} \) \\ \( P_n(x;a,b,c|q) \) \end{tabular} & |(23)| \begin{tabular}{c} \( \text{Big -1 Jacobi} \) \\ \( J_n(x;\alpha,\beta,c) \) \end{tabular} \\
|(31)| \begin{tabular}{c} \( \begin{array}{c}
       \text{Generalized}\\\text{Gegenbauer}
      \end{array} \) \\ \( G_n(x;\alpha,\beta) \) \end{tabular} & |(32)| \begin{tabular}{c} \( \text{Little q-Jacobi} \) \\ \( P_n(x;b,a|q) \) \end{tabular} & |(33)| \begin{tabular}{c} \( \text{Little -1 Jacobi} \) \\ \( P_n(x;\alpha,\beta) \) \end{tabular} \\
|(41)| \begin{tabular}{c} \( \text{Gegenbauer} \) \\ \( G_n(x;\beta+\frac{1}{2}) \) \end{tabular} & |(42)| \begin{tabular}{c} \( \begin{array}{c}
       \text{Special}\\\text{Little q-Jacobi}
      \end{array} \) \\ \( P_n(x;b|q) \) \end{tabular} & |(43)| \begin{tabular}{c} \( \begin{array}{c}
       \text{Special}\\\text{Little -1 Jacobi}
      \end{array} \) \\ \( P_n(x;\beta) \) \end{tabular} \\
|(51)| \begin{tabular}{c} \( \text{Legendre} \) \\ \( L_n(x) \) \end{tabular} & |(52)|  & |(53)| \begin{tabular}{c} \( \begin{array}{c}
3^{\text{rd}} \text{kind}\\\text{Chebyshev}
\end{array} \) \\ \( T_n(x) \) \end{tabular} \\      
};
\tikzstyle{every node}=[font=\small\itshape]
\draw (22) -- node[midway,right] {$c\to 0$}(32);
\draw (21) -- node[midway,right] {$\gamma\to 0$}(31);
\draw (23) --  node[midway,right] {$c\to 0$}(33);
\draw (22) -- node[midway,above] {$q\to-1$} (21);
\draw (32) -- node[midway,above] {$q\to-1$} (31);
\draw (22) -- node[midway,above] {$q\to-1$} (23);
\draw (32) -- node[midway,above] {$q\to-1$} (33);
\draw (42) -- node[midway,above] {$q\to-1$} (41);
\draw (42) -- node[midway,above] {$q\to-1$} (43);
\draw (32) -- node[midway,right] {$a\to -1$}(42);
\draw (31) -- node[midway,right] {$\alpha\to -\frac{1}{2}$}(41);
\draw (33) --  node[midway,right] {$\alpha\to 0$}(43);
\draw (41) -- node[midway,right] {$\beta\to 0$}(51);
\draw (43) --  node[midway,right] {$\beta\to 0$}(53);
\end{tikzpicture}}\end{center}
